Safe and Efficient Path Planning under Uncertainty via Deep Collision Probability Fields

Estimating collision probabilities between robots and environmental obstacles or other moving agents is crucial to ensure safety during path planning. This is an important building block of modern planning algorithms in many application scenarios such as autonomous driving, where noisy sensors perceive obstacles. While many approaches exist, they either provide too conservative estimates of the collision probabilities or are computationally intensive due to their sampling-based nature. To deal with these issues, we introduce Deep Collision Probability Fields, a neural-based approach for computing collision probabilities of arbitrary objects with arbitrary unimodal uncertainty distributions. Our approach relegates the computationally intensive estimation of collision probabilities via sampling at the training step, allowing for fast neural network inference of the constraints during planning. In extensive experiments, we show that Deep Collision Probability Fields can produce reasonably accurate collision probabilities (up to 10^{-3}) for planning and that our approach can be easily plugged into standard path planning approaches to plan safe paths on 2-D maps containing uncertain static and dynamic obstacles. Additional material, code, and videos are available at https://sites.google.com/view/ral-dcpf.

==> img/experiments/01_network_evaluation/rmsre_barplot.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
    bin & min & max & mean \\
    {[0, 0.001[}    & 0.90709388256073 & 8.347548484802246 & 1.3494278192520142        \\
    {[0.001, 0.01[} & 0.02559514530003071 & 0.4587242007255554 & 0.0656203031539917    \\
    {[0.01, 0.1[}   & 0.014518298208713531 & 0.30218496918678284 & 0.03820294886827469 \\
    {[0.1, 1]}      & 0.008359751664102077 & 0.12974144518375397 & 0.02331957221031189 \\
    {[0, 1]}        & 0.4875592589378357 & 4.491858005523682 & 0.7258647680282593      \\
}\binrrmsedata


\begin{figure}[t]
\centering
%\includegraphics[width=0.5\textwidth]{figures/experiments/binrrmse.png}
\begin{tikzpicture}
    \begin{axis}[
            ybar,
            % ymode=log,
            bar width=.5cm,
            width=0.89\textwidth,
            height=.30\textwidth,
            legend style={at={(1,1)},
                anchor=east,legend columns=-1},
            symbolic x coords={{[0, 0.001[},{[0.001, 0.01[},{[0.01, 0.1[},{[0.1, 1]},{[0, 1]}},
            xtick=data,
            major tick length=0cm,
            nodes near coords,
            every node near coord/.append style={rotate=90, anchor=west},
            %nodes near coords align={vertical},
            ymin=0,ymax=2,
            ylabel={Root Mean Squared Relative Error},
            xlabel={Intervals of Ground Truth}% ,
            %cycle list name=Dark2-3
        ]
        \addplot table[x=bin,y=mean]{\binrrmsedata};
        \addplot table[x=bin,y=min]{\binrrmsedata};
        \addplot table[x=bin,y=max]{\binrrmsedata};
        \legend{Mean, Single (Best), Single (Worst)}
    \end{axis}
\end{tikzpicture}



\caption{Bar Plot of RMSRE evaluated on test dataset (Will probably not be used)}
\label{fig:binrrmse}
\end{figure}

==> old/experiments/binrrmse.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
    bin & mean & single \\
    0.0001  & 6.5112376e-04 & 6.9669477e-04  \\
    0.001   & 2.3514552e-04 & 2.8522228e-04  \\
    0.01    & 6.3600106e-05 & 9.3361232e-05  \\
    0.1     & 4.9874299e-05 & 5.4017182e-05  \\
    0.5     & 1.4626316e-05 & 1.6891951e-05  \\
    1       & 3.8588470e-07 & 7.8782131e-07  \\
    }\binrrmsedata



\begin{tikzpicture}
    \begin{axis}[
            ybar,
            bar width=.5cm,
            width=.48\textwidth,
            %height=.5\textwidth,
            legend style={at={(0.79,1)},
                anchor=north,legend columns=-1},
            symbolic x coords={0.0001,0.001,0.01,0.1,0.5,1},
            major tick length=0cm,
            xtick=data,
            nodes near coords,
            every node near coord/.append style={rotate=90, anchor=west},
            %nodes near coords align={vertical},
            ymin=0,ymax=0.001,
            ylabel={RRMSE},
            xlabel={Upper Bound of Bin}
        ]
        \addplot table[x=bin,y=mean]{\binrrmsedata};
        \addplot table[x=bin,y=single]{\binrrmsedata};
        \legend{Mean, Single}
    \end{axis}
\end{tikzpicture}

==> old/experiments/pred-gt_max_cp_0.1.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
    state & mean & meanci & max \\
%    3&     1.976197e-14  &  3.586020e-14  &  5.928591e-14 \\
%    4&     5.743869e-07  &  9.078534e-07  &  1.521067e-06 \\
    5&     -4.342874e-03 & -1.279798e-04  &  2.872786e-03 \\
    6&     2.980693e-04  &  9.555643e-03  &  2.311063e-02 \\
    7&     -2.877791e-03 &  7.099416e-03  &  2.498612e-03 \\
    8&     -5.478974e-03 & -4.087128e-03  &  9.932531e-03 \\
    9&     3.794304e-04  &  5.581457e-04  &  3.442627e-05 \\
    10&     -8.551170e-03 & -7.161442e-03  &  1.895290e-03 \\
%    11&     3.551018e-03  &  5.625328e-03  &  5.331697e-03 \\
    }\ensemblecompdata


%\includegraphics[width=0.5\textwidth]{figures/experiments/pred-gt_max_cp_0.1.png}
\begin{tikzpicture}
    \begin{axis}[
            ybar,
            bar width=.5cm,
            width=.49\textwidth,
            height=.5\textwidth,
            legend style={at={(.7,1)},
                anchor=north,legend columns=-1},
            symbolic x coords={5,6,7,8,9,10},
            major tick length=0cm,
            bar width = 7pt,
            xtick=data,
            visualization depends on=y\as\myy,
            nodes near coords,
            nodes near coords style = {anchor ={90+sign(\myy)*90}},
            every node near coord/.append style={rotate=90},
            %nodes near coords align={vertical},
            ymin=-0.03,ymax=0.04,
            ylabel={$\hat{y}-y$},
            xlabel={State}
        ]
        \addplot table[x=state,y=mean]{\ensemblecompdata};
        \addplot table[x=state,y=meanci]{\ensemblecompdata};
        \addplot table[x=state,y=max]{\ensemblecompdata};
        \legend{mean, mean+ci, max}
    \end{axis}
\end{tikzpicture}

==> old/experiments/tiago_contour_plot.tex <==
\begin{figure}
\centering
\begin{tabular}{cc}
  \includegraphics[width=.2\textwidth]{figures/experiments/tiago_12.png} &  \includegraphics[width=.2\textwidth]{figures/experiments/tiago_40.png} \\
\includegraphics[width=.2\textwidth]{figures/experiments/tiago_collision_z_12.png}  & \includegraphics[width=.2\textwidth]{figures/experiments/tiago_collision_z_40.png}   \\[6pt]
% \includegraphics[width=65mm]{it} &   %\includegraphics[width=65mm]{figures/experiments/exp2_ci_0.001.png} \\
%(c) third & (d) fourth \\[6pt]
\end{tabular}
\caption{Collision probability estimates from single trained ReDCPF for two different joint configurations.}
\label{fig:tiago_collisions}
\end{figure}

==> sections/data_generation.tex <==
\subsection{Data generation}
\label{sec:data-gen}
We resort to a sampling-based method to generate an accurate dataset that does not leverage approximations to compute CPs. Specifically, since we are not bound by time constraints at this stage, we resort to Simple Monte Carlo sampling. %\footnote{More sophisticated methods, like those based on importance sampling, could in principle be used to reduce the dataset generation time and scale the approach to smaller CPs.} 
Another key observation is that the desired accuracy of the \gls{cp} estimate directly depends on the \gls{cp} itself. For example, suppose that after having drawn 10k samples, our current \gls{cp} estimate is .5; in this case, we would accept an error of .01, especially if our planning constraint $p_{\text{max}}$  is .01 or .1. Following from this observation, we define the following probability intervals: $[0, .01)$, $[.01, .1)$, $[.1, 1]$. Each interval is then associated with a different desired accuracy for a \gls{clt} based 95\% confidence interval estimate\footnote{See~\cite{mcbook}, Eq. (2.20), and the following paragraph for the special case of estimated \gls{cp} = 0 or 1.}: $\pm.01$, $\pm.001$, $\pm10^{-4}$. Therefore, we can stop drawing samples as soon as the current \gls{clt}-based 95\% confidence interval falls below the accuracy associated with the current \gls{cp} estimate. To speed up this procedure, we only recompute the \gls{cp} estimate and associated confidence interval after having drawn a batch of samples. We use batches of $4\cdot 10^4$ samples, and $4\cdot 10^6$ maximum total samples, computed as the worst-case number of samples needed for the smallest probability interval. 

Another issue to consider during the training is to sample properly the robot configurations to be evaluated. Indeed, if the dataset size is a concern, sampling uniformly may require a prohibitively large amount of samples to properly cover the areas where the estimation of collision probability is particularly sensible. 
We propose a sampling method based on the \gls{minsum} between the robot and the obstacle. The \gls{minsum} is the shape obtained by sliding the robot shape around the obstacle~\cite{claes_collision_2012}. 
Our key idea is to compute a shape that resembles the isolines of the \gls{cp} landscape, particularly close to the constraint budget level, and subsequently sample points from it.
In a scenario without uncertainty, this shape can be trivially obtained by computing the \gls{minsum} between the robot and the obstacle. To take the uncertainties $\mSigma_o=(\sigma_x,\sigma_y,\sigma_{\phi},\sigma_{l_1},\sigma_{l_2})$ into account we apply various strategies. 
For positional and shape variance we construct an inflated shape $s_\text{inflated}$ by computing a \gls{minsum} between the shape of the obstacle $s_o$ and an ellipse $s_e \sim N(\sigma_x + \sigma_{l_1}, \sigma_y +\sigma_{l_2} | \left(\sigma_x + \sigma_{l_1}, \sigma_y +\sigma_{l_2}\right))$.
% The effects of rotational variance are approximated by a union $s_u$ of $s_{ps}$ for rotated obstacles $s_o$. The rotations are a discretization of the interval  $[-\phi_m, \phi_m]$ with $\phi_m \sim \mathcal{U}(\sigma_\theta, 3.1\cdot\sigma_\theta)$.
% In our experiment, we found that three rotations are sufficient if we apply some smoothing, by growing and shrinking $s_u$.
The effects of rotational variance are approximated by constructing the shape $s_\text{rotational}$, by computing the union of multiple $s_\text{inflated}$ for rotated obstacles $s_o$. On top of that, we smooth the obtained shape by growing and shrinking $s_\text{rotational}$. The rotations are a discretization of the interval  $[-\phi_m, \phi_m]$ with $\phi_m \sim \mathcal{U}(\sigma_\theta, 3.1\cdot\sigma_\theta)$.
In our experiment, we found that three rotations are sufficient, for this heuristic to result in sample configurations for a well-balanced dataset.

==> tables/network_ablation_rmsre.tex <==
%\footnotesize
%\begin{tabular}{l|ccccc}
%\hline
%Network & $[10^{-4}, 10^{-3})$ & $[10^{-3}, 10^{-2})$ & $[10^{-2}, 10^{-1})$ & $[10^{-1}, 1]$ & $[10^{-4}, 1]$ \\ \hline
%128x3  & $2.032$ & $3.730\cdot10^{-1}$ & $8.756\cdot10^{-2}$ & $3.078\cdot10^{-2}$ & $7.342\cdot10^{-1}$ \\
%512x3  & $1.274$ & $2.594\cdot10^{-1}$ & $7.125\cdot10^{-2}$ & $2.815\cdot10^{-2}$ & $4.638\cdot10^{-1}$ \\
%512x4  & $3.737$ & $5.495\cdot10^{-1}$ & $9.321\cdot10^{-2}$ & $2.717\cdot10^{-2}$ & $1.335$\\
%1024x4 & $0.940$ & $1.864\cdot10^{-1}$ & $5.157\cdot10^{-2}$ & $2.393\cdot10^{-2}$ & $3.418\cdot10^{-1}$ \\
%1024x5 & $\mathbf{0.788}$ & $\mathbf{1.684\cdot10^{-1}}$ & $\mathbf{4.998\cdot10^{-2}}$ & $2.246\cdot10^{-2}$ & $\mathbf{2.885\cdot10^{-1}}$ \\
%1024x6 & $1.287$ & $2.537\cdot10^{-1}$ & $6.583\cdot10^{-2}$ & $2.430\cdot10{-2}$ & $4.674\cdot10^{-1}$ \\
%1024x7 & $0.964$ & $1.808\cdot10^{-1}$ & $5.144\cdot10^{-2}$ & $\mathbf{2.228\cdot10{-2}}$ & $3.494\cdot10^{-1}$ \\
%\hline
%\end{tabular}
%\normalsize

\footnotesize
\begin{tabular}{l|cccc}
\hline
Network &  $[10^{-3}, 10^{-2})$ & $[10^{-2}, 10^{-1})$ & $[10^{-1}, 1]$ & $[10^{-3}, 1]$ \\ \hline
3x128 & $0.330948$ & $0.078886$ & $0.027899$ & $0.163615$ \\
3x512 & $0.465704$ & $0.088191$ & $0.028413$ & $0.226027$ \\
4x512 & $0.218781$ & $0.057394$ & $0.023245$ & $0.109486$ \\
4x1024 & $0.208752$ & $0.056301$ & $0.023988$ & $0.104925$ \\
5x1024 & $0.214154$ & $0.057572$ & $0.022780$ & $0.107434$ \\
6x1024 & $\mathbf{0.183206}$ & $\mathbf{0.050278}$ & $\mathbf{0.022065}$ & $\mathbf{0.092351}$ \\
7x1024 & $0.183474$ & $0.053021$ & $0.022736$ & $0.093079$ \\
\hline
\end{tabular}
\normalsize



==> tables/random_obstacles_results.tex <==
% \footnotesize
% \begin{tabular}{p{1.8cm}|rrrrrrr} % Set the leftmost column width to 4cm
%     \hline
%     \multirow{2}{*}{Metric} 
%     & \multirow{2}{*}{DCPF} & $z$-Test    & $z$-Test    & $z$-Test & $z$-Test    & $z$-Test  & \multirow{2}{*}{SPRT}  \\
%     &                       & \tiny $n=10$      & \tiny  $n=100$     & \tiny  \tiny $n=1000$ & \tiny  $n=10000$   & \tiny  $n=50000$ &  \\ \hline
%     No solution & 24 & \22 & 23 & 23 &  24 & 48 & 24  \\
%     Violations &  \textbf{2} & 26 & 18 & 3  & \textbf{2} & 3 & \textbf{2} \\
%     Violations $>$ CI &  \textbf{0} & 26 & 18 & 3 & 2 & 3 & -\\
%     \multirow{2}{2cm}{\gls{mae} $(\cdot 10^{-2})$} &  \textbf{0.0003} & 0.2128 & 0.0094 & 0.0009 & 0.0009 & 0.0008 & -   \\
%     &  \textbf{$\pm$0.0060} & $\pm$1.5307 & $\pm$0.0720 & $\pm$0.0077 & $\pm$0.0070 & $\pm$0.0070 & - \\
%     \multirow{2}{2cm}{Mean violation $(\cdot 10^{-2})$} &  \textbf{0.1439} & 4.5444 & 0.4035 & 0.1496  & 0.1459 & 0.1260 & -  \\
%     &  \textbf{$\pm$0.1348} & $\pm$5.5183 & $\pm$0.2933 & $\pm$0.0159 & $\pm$0.0093 & $\pm$0.0236 & - \\
%     \multirow{2}{2cm}{Mean path length [m]} & 28.9868 & 29.0769 & 29.1299 & 29.2078 & 28.8816 &  \textbf{27.5769} & 28.7895 \\
%     & $\pm$4.2037 & $\pm$4.8563 & $\pm$4.9316 & $\pm$4.9657 & $\pm$4.3346 & \textbf{$\pm$3.8548} & $\pm$4.2960 \\
%     Mean t [min] &  \textbf{0.6616} & 2.3799 & 2.4611 & 3.8731 & 7.3175 & 7.3116 & 6.7175  
% \end{tabular}
% \normalsize




% \footnotesize
% \begin{tabular}{p{1.8cm}|rrrrrrr} % Set the leftmost column width to 4cm
%     \hline
%     \multirow{2}{*}{Metric} 
%     & \multirow{2}{*}{DCPF} & $z$-Test    & $z$-Test    & $z$-Test & $z$-Test    & $z$-Test  & \multirow{2}{*}{SPRT}  \\
%     &                       & \tiny $n=10$      & \tiny  $n=100$     & \tiny  \tiny $n=1000$ & \tiny  $n=10000$   & \tiny  $n=50000$ &  \\ \hline
%     No solution & 69 & 64 & 69 & 71 & 76 & 106 & 73  \\
%     % Violations &  8 & 146 & 43 & 10 & 8 & 10 & 7 \\
%     % Violations $>$ CI & 1 & 145 & 43 & 10 & 5 & 9 & 7\\
%     Violations & 1 & 145 & 43 & 10 & 5 & 9 & 7\\
%     Not decidable &  7 & 1 & 0 & 0 & 3 & 1 & 0 \\
%    % \multirow{2}{2cm}{\gls{mae} $(\cdot 10^{-2})$} & 0.0013 & 0.1158 & 0.0289 & 0.0218 & 0.0221 & 0.0207 & -   \\
%    % & $\pm$0.0174 & $\pm$0.9884 & $\pm$0.3093 & $\pm$0.2321 & $\pm$0.2262 & $\pm$0.1919 & - \\
%     % \multirow{2}{2cm}{Mean violation $(\cdot 10^{-2})$} &  \textbf{0.1439} & 4.5444 & 0.4035 & 0.1496  & 0.1459 & 0.1260 & -  \\
%     % &  \textbf{$\pm$0.1348} & $\pm$5.5183 & $\pm$0.2933 & $\pm$0.0159 & $\pm$0.0093 & $\pm$0.0236 & - \\
%     \multirow{2}{2cm}{Mean path length [m]}& 29.2554 & 29.2500 & 29.3636 & 29.2183 & 28.9688 & 28.6392 & 29.1013 \\
%     & $\pm$5.1815 & $\pm$4.9370 & $\pm$5.2815 & $\pm$5.0227 & $\pm$4.6468 & $\pm$4.3261 & $\pm$4.7975 \\
%     %Mean t [ms]  & 39.1800 & 1.1863 & 1.2524 & 1.2068 & 1.2083 & 1.2089 & 13.7464
% \end{tabular}
% \normalsize

% \small
% \begin{tabular}{p{1.8cm}|rrrrrrr} % Set the leftmost column width to 4cm
%     \hline
%     \multirow{2}{*}{Metric} 
%     & \multirow{2}{*}{DCPF} & $z$-Test    & $z$-Test    & $z$-Test & $z$-Test    & $z$-Test  & \multirow{2}{*}{SPRT}  \\
%     &                       & \tiny $n=10$      & \tiny  $n=100$     & \tiny  \tiny $n=1000$ & \tiny  $n=10000$   & \tiny  $n=50000$ &  \\ \hline
%     No solution & 69 & 73 & 73 & 70 & 94 & 145 & 94  \\
%     Violations & 0 & 756 & 232 & 60 & 22 & 24 & 22\\
%     Not decidable & 10 & 0 & 0 & 0 & 0 & 2 & 0 \\
%     \multirow{2}{2cm}{Mean path length [m]}& 33.1775 & 32.9692 & 32.9515 & 33.1696 & 32.6505 & 32.0710 & 32.7561\\
%     & $\pm$4.8491 & $\pm$4.9557 & $\pm$4.5408 & $\pm$4.8564 & $\pm$4.1658 & $\pm$3.5598 & $\pm$4.2079 \\
% \end{tabular}
% \normalsize
% \footnotesize
% \begin{tabular}{p{1.8cm}|rrrr} % Set the leftmost column width to 4cm
%     \hline
%     \multirow{2}{*}{Metric} 
%     & \multirow{2}{*}{DCPF} & $z$-Test    & $z$-Test    & $z$-Test   \\
%     &                       & \tiny $n=10$      & \tiny  $n=100$     & \tiny  \tiny $n=1000$ \\ \hline
%     No solution & \textbf{69} & 73 & 73 & 70 \\
%     Violations & \textbf{0} & 756 & 232 & 60 \\
%     Not decidable & 10 & 0 & 0 & 0  \\
%     \multirow{2}{2cm}{Mean path length [m]}& 33.1775 & 32.9692 & 32.9515 & 33.1696\\
%     & $\pm$4.8491 & $\pm$4.9557 & $\pm$4.5408 & $\pm$4.8564 \\
%     \hline

%     \multirow{2}{*}{Metric} & $z$-Test    & $z$-Test  & \multirow{2}{*}{SPRT} \\
%     & \tiny  $n=10000$   & \tiny  $n=50000$ & \\ \hline
%     No solution & 94 & 145 & 94  \\
%     Violations & 22 & 24 & 22\\
%     Not decidable & 0 & 2 & 0 \\
%     \multirow{2}{2cm}{Mean path length [m]} & 32.6505 & \textbf{32.0710} & 32.7561\\
%     & $\pm$4.1658 & \textbf{$\pm$3.5598} & $\pm$4.2079 \\
%     \hline
% \end{tabular}
% \normalsize


\footnotesize
\begin{tabular}{p{1.8cm}|rrrr} % Set the leftmost column width to 4cm
    \hline
    \multirow{2}{*}{Metric} 
    & \multirow{2}{*}{DCPF} & $z$-Test    & $z$-Test    & $z$-Test   \\
    &                       & \tiny $n=100$      & \tiny  $n=1000$     & \tiny  \tiny $n=10000$ \\ \hline
    No solution & 69 & 223 & 144 & 72 \\
    \multirow{2}{2cm}{Mean path length [m]}& 33.1775 & 33.0779 & 33.3846 & 33.0702\\
    & $\pm$4.8491 & $\pm$4.8316 & $\pm$5.6823 & $\pm$4.8236 \\
    Time[s] & 122.9647 & 11.9174 & 22.9959 & 114.7412 \\
    \hline 

    \multirow{2}{*}{Metric} & $z$-Test    & $z$-Test   & $z$-Test  & SPRT \\
    & \tiny  $n=1e5$   & \tiny  $n=1e6$ & \tiny  $n=4e6$ & \tiny  $n=4e6$\\ \hline
    No solution & 72 & 71 & 71 & 65 \\
    \multirow{2}{2cm}{Mean path length [m]} & 33.0702 & 33.0957 & 33.1135 & 33.3702\\
    & $\pm5.0214$& $\pm$5.1177 & $\pm$5.1217 & $\pm$5.2830 \\
    Time[s] & 191.0387 & 1086.9447 & 3932.4689 & 109.6519 \\
    \hline
\end{tabular}
\normalsize
